SPOCK: A proximal method for multistage risk-averse optimal control problems

Risk-averse optimal control problems have gained a lot of attention in the last decade, mostly due to their attractive mathematical properties and practical importance. They can be seen as an interpolation between stochastic and robust optimal control approaches, allowing the designer to trade-off performance for robustness and vice-versa. Due to their stochastic nature, risk-averse problems are of a very large scale, involving millions of decision variables, which poses a challenge in terms of efficient computation. In this work, we propose a splitting for general risk-averse problems and show how to efficiently compute iterates on a GPU-enabled hardware. Moreover, we propose Spock - a new algorithm that utilizes the proposed splitting and takes advantage of the SuperMann scheme combined with fast directions from Anderson's acceleration method for enhanced convergence speed. We implement Spock in Julia as an open-source solver, which is amenable to warm-starting and massive parallelization.

==> parts_arXiv/approx_optimal_points.tex <==
Let us introduce the notion of an approximate optimal point, $z^\star$, that is, a point that satisfies the optimality condition of Equation \eqref{eq:optimality-condition} approximately in the following sense.
\begin{definition}[Approximate optimal point]
A point $\tilde{z}$ is an $\epsilon$-approximate point for $\mathbb{P}$ if there is $\xi_0$ with $\|\xi_0\|_\infty \leq \epsilon$ such that 
\begin{equation}
    \xi_0 \in \partial f(\tilde{z}) + L^* \partial g(L \tilde{z}).
\end{equation}
\end{definition}
By writing $\xi_0 = \xi_1 + L^* \xi_2$ we can see that a point $\tilde{z}$ is an $\epsilon$-approximate point for $\mathbb{P}$ if there is an $\tilde{\eta}$ such that
\begin{subequations}\label{eq:approx-primal-dual-point}
\begin{align}
    \xi_1 \in \partial f(\tilde{z}) + L^* \tilde{\eta},
    \label{eq:approx-primal-dual-point:a}
    \\
    \tilde{\eta} + \xi_2 \in \partial g(L \tilde{z}).
    \label{eq:approx-primal-dual-point:b}
\end{align}
\end{subequations}
This allows us to introduce a notion of approximate primal-dual optimality.
\begin{definition}[Approximate primal-dual optimality]
A point $(\tilde{z}, \tilde{\eta})$ is said to be an $\epsilon$-approximate primal-dual optimal point for $\mathbb{P}$ if it satisfies the conditions of Equation \eqref{eq:approx-primal-dual-point} with $\|\xi_1\|_\infty\leq\epsilon$, $\|\xi_2\|_\infty\leq\epsilon$ and $\|\xi_1 + L^* \xi_2\|_\infty \leq \epsilon$.
\end{definition}
We need to propose conditions under which an iterate $(z_k, \eta_k)$ of the Chambolle-Pock algorithm is an $\epsilon$-approximate primal-dual point. Since the Chambolle-Pock algorithm involves $g^*$, it is useful to introduce a regularity assumption \cite[]{ioffe_metric-regularity} for $\partial g^*$ that will allow us to argue that the satisfaction of an approximate optimality condition that involves $\partial g$ --- as in Equation \eqref{eq:approx-primal-dual-point:b} --- implies that a condition akin to Equation \eqref{eq:primal-dual-point:b} is satisfied approximately. To that end, we state the following assumption:
\begin{assumption}
Suppose that the Chambolle-Pock method converges to a pair $(z^\star, \eta^\star)$ with $(\eta^\star, L z^\star)\in \gph \partial g^*$. We assume that $\partial g^*$ is metrically regular with modulus $\tau$ at $(\eta^\star, L z^\star)$, that is, there is $r>0$ such that 
\begin{equation}
    d(\eta, \partial g(L z)) \leq \tau d(L z, \partial g^*(\eta)),
\end{equation}
for $\|\eta-\eta^\star\|\leq r$ and $\|L z - L z^\star\|\leq r$.
\end{assumption}
Under the above assumption, if we can determine a pair $(z, \eta)$ such that $d(L z, \partial g^*(\eta)) \leq \epsilon/\tau$, it follows that the condition of Equation \eqref{eq:approx-primal-dual-point:b} is satisfied for some $\xi_2$ with $\|\xi_2\|_\infty \leq \epsilon$. This leads to the following result

\begin{proposition}
A pair $(\tilde{z}, \tilde{\eta})$ is an $\epsilon$-approximate optimal point if there are $\xi_1$ and $\xi_2$ with $\|\xi_1\|_\infty \leq \epsilon$ and $\|\xi_2\|_\infty\leq \epsilon/\tau$ and $\|\xi_1 + L^*\xi_2\|_\infty\leq \epsilon$ such that 
\begin{subequations}
\begin{align}
    \xi_1 \in L^* \tilde{\eta} + \partial f(\tilde{z}),
    \label{eq:xi1_intro}
    \\
    L \tilde{z} + \xi_2 \in \partial g^*(\tilde{\eta}).
    \label{eq:xi2_intro}
\end{align}
\end{subequations}
\end{proposition}


\subsubsection{Termination criteria}
In this section we state conditions under which we can guarantee that an iterate of the Chambolle-Pock algorithm is an approximate optimal point in the sense defined above. We use \eqref{eq:cp-primal} and \eqref{eq:xi1_intro} to define
\begin{equation}
    \xi_1^{k+1} {}:={} \dfrac{z_k - z_{k+1}}{\alpha_1} - L^*\left(\eta_k - \eta_{k+1}\right),
\end{equation}
and similarly, we use \eqref{eq:cp-dual} and \eqref{eq:xi2_intro} to define
\begin{equation}
    \xi_2^{k+1} {}:={} \dfrac{\eta_k - \eta_{k+1}}{\alpha_2} + L\left(z_{k+1} - z_k\right).
\end{equation}

Thus the termination criteria are $\|\xi_1^{k+1}\|_\infty \leq \epsilon$, $\|\xi_2^{k+1}\|_\infty \leq \epsilon/\tau$, and $\|\xi_1^{k+1} + L^* \xi_2^{k+1}\|_\infty \leq \epsilon$. Once the termination criteria are satisfied, we return $(z_{k+1}, \eta_{k+1})$ which is an $\epsilon$-approximate optimal point. This will happen as $z_k \to z^\star$ and $\eta_k \to \eta^\star$, provided there is a fixed point of the Chambolle-Pock method. In practice, it may not always be possible to determine $\tau$.



==> parts_arXiv/approx_solutions.tex <==
\subsection{Approximate optimal points}
\subsubsection{Preliminaries}
In what follows, $d$ denotes a point-to-set distance and for a multifunction $G:X\rightrightarrows Y$ we denote its graph by $\gph G = \{(x, y): y \in G(x)\}$.

\begin{definition}[Metric regularity]
A multifunction $G:\R^n\rightrightarrows \R^n$ is said to be metrically regular near $(\bar{x}, \bar{y})\in\gph G$ with modulus $\tau>0$ if there is an $\epsilon>0$ such that 
\begin{equation}
    d(x, G^{-1}(y))\leq \tau d(y, G(x)),
\end{equation}
for all $(x,y)$ that are $\epsilon$-close to $(\bar{x}, \bar{y})$.
\end{definition}
To say that $\partial g^*$ is metrically regular at $(\bar{x}, \bar{y})\in\gph \partial g^* \Leftrightarrow \bar{x} \in \partial g^*(\bar{y})$ means that 
\begin{equation}
    d(x, \partial g(y))\leq \tau d(y, \partial g^*(x)),
\end{equation}
for all $(x,y)$ that are $\epsilon$-close to $(\bar{x}, \bar{y})$.



==> parts_arXiv/preamble.tex <==
\RequirePackage[mathscr]{euscript}
\RequirePackage[utf8]{inputenc}
\RequirePackage{amssymb,amsmath,amsfonts,mathtools}
\RequirePackage{hhline}
\RequirePackage{algorithm}
\RequirePackage{nicefrac}
\RequirePackage{soul,color} %
\RequirePackage{xargs}
\RequirePackage{datetime}
\RequirePackage{bm}
\RequirePackage[table,usenames,dvipsnames]{xcolor}

\newcommand{\SPOCK}{\textsc{Spock}}
\newcommand{\MOSEK}{\textsc{Mosek}}
\newcommand{\GUROBI}{\textsc{Gurobi}}
\newcommand{\COSMO}{\textsc{Cosmo}}
\newcommand{\IPOPT}{\textsc{Ipopt}}
\newcommand{\SEDUMI}{\textsc{Sedumi}}
\newcommand\mymathbb[1]
{ {\rm I\mathchoice{\hspace*{-2pt}}{\hspace*{-2pt}}
      {\hspace*{-1.75pt}}{\hspace*{-1.7pt}}#1}   }        %
\newcommand{\R}{\mymathbb R}				%
\newcommand{\N}{\mymathbb N}				%
\newcommand{\dd}{\mathrm{d}}				%
\newcommand{\C}{\mathbb{C}}
\newcommand{\ttop}{{\scalebox{.75}{$\scriptscriptstyle \top$}}}
\newcommand{\dom}{\operatorname{\mathbf{dom}}}
\newcommand{\smallplus}{{\scriptscriptstyle +}}
\newcommand{\Spp}{\mathbb{S}_{\smallplus\smallplus}}
\newcommand{\Sp}{\mathbb{S}_{\smallplus}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\blkdiag}{\operatorname{blkdiag}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\rank}{\operatorname{\mathbf{rank}}}
\newcommand{\lev}{\operatorname{\mathbf{lev}}}
\newcommand{\epi}{\operatorname{\mathbf{epi}}}
\newcommand{\prox}{\operatorname{\mathbf{prox}}}
\newcommand{\ocp}{\mathbb{P}}
\DeclareMathOperator*{\argmin}{\mathbf{arg\,min}}
\DeclareMathOperator*{\argmax}{\mathbf{arg\,max}}
\DeclareMathOperator*{\minimise}{\mathbf{minimize}}
\DeclareMathOperator*{\minimize}{\mathbf{minimize}}
\newcommand{\dfn}{\mathrel{\mathop:}=}
\newcommand{\smallmat}[1]{\left[ \begin{smallmatrix}#1           \end{smallmatrix} \right]}
\newcommand{\rn}[1]{{\rm \MakeUppercase{\romannumeral #1}}}
\newcommand\smashunderbracket[3][0.5pt]{%
  \vphantom{#2}%
  \smash{\underbracket[#1]{#2}_{#3}}%
}


\RequirePackage{booktabs} %
\RequirePackage{pgfplots}
\usepackage{units}
\usepackage[noend]{algpseudocode}
\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing,
  patterns,arrows,positioning, backgrounds, intersections}
\tikzstyle{Nodes}=[circle, draw=black, fill=red!30, line width=0.7pt, minimum size=20pt]
\tikzstyle{arrow} = [line width=1pt,->,>=stealth]
\tikzstyle{axis} = [line width=1pt,->,>=stealth]
\usepackage{tcolorbox}
\usepackage{framed}
\usepackage{mdframed}
\usepackage{marvosym}
\usepackage{tabularx,array,xspace}
\usepackage[makeroom]{cancel}
\usepackage{romanbar}
\usepackage{hyperref}
\hypersetup{
  unicode=false,          %
  pdftoolbar=true,        %
  pdfmenubar=true,        %
  pdffitwindow=false,     %
  pdfstartview={FitH},    %
  pdftitle={notes},    %
  pdfauthor={},                %
  pdfsubject={optimal control},                   %
  pdfcreator={LaTeX},                            %
  pdfproducer={},      %
  pdfkeywords={BotDozer},      %
  pdfnewwindow=true,      %
  colorlinks=true,        %
  linkcolor=blue!90,    %
  citecolor=red,         %
  filecolor=magenta,      %
  urlcolor=NavyBlue           %
}

\mathtoolsset{centercolon}
\newcommand{\E}{{\rm I\!E}}
\newcommand{\mytop}{{\scalebox{.75}{$\scriptscriptstyle \top$}}}
\newcommand{\Rext}{\overline{\R}}
\newcommand{\ellb}{\bar{\ell}}
\newcommand{\Vb}{{\overline{V}}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\Top}{^\intercal}
\newcommand{\iTop}{^{i\intercal}}
\newcommand{\jTop}{^{j\intercal}}
\newcommand{\proj}{\operatorname{\mathbf{proj}}}
\newcommand{\AVaR}{\operatorname{AV@R}}
\newcommand{\essmax}{\operatorname{essmax}}
\let\oldmax\max
\renewcommand{\max}{\bm{\oldmax}}
\let\oldmin\min
\renewcommand{\min}{\bm{\oldmin}}
\let\oldinf\inf
\renewcommand{\inf}{\bm{\oldinf}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\xb}{\bar{x}}
\newcommand{\ub}{\bar{u}}
\newcommand{\yb}{\bar{y}}
\renewcommand{\sb}{\bar{s}}
\newcommand{\tb}{\bar{\tau}}
\newcommand{\zb}{\bar{z}}
\newcommand{\nb}{\bar{\eta}}
\newcommand{\Ab}{\bar{A}}
\newcommand{\gph}{\operatorname{\mathbf{gph}}}
\newcommand{\SOC}{\operatorname{SOC}}
\newcommand{\ri}{\mathbf{ri}}
\newcommand{\fix}{\mathbf{fix}\text{ }}
\newcommand{\id}{\mathrm{id}}

\makeatletter
\renewcommand*\env@matrix[1][c]{\hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols #1}}
\makeatother

\definecolor{myred}{rgb}{1,0,0}
\definecolor{mygreen}{rgb}{.3,.8,0}
\definecolor{myblue}{rgb}{0,0,1}
\definecolor{myyellow}{rgb}{.9,.7,0}
\definecolor{mypurple}{rgb}{.9,0,.7}

\newcommand{\nodes}{\operatorname{\mathbf{nodes}}}
\newcommand{\ch}{\operatorname{\mathbf{ch}}}
\newcommand{\anc}{\operatorname{\mathbf{anc}}}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{assumption}[theorem]{Assumption}

\newcommand{\pantelis}[1]{{\color{mypurple}#1}}
\newcommand{\ruairi}[1]{{\color{mygreen}#1}}
\newcommand{\mathijs}[1]{{\color{myyellow}#1}}
\newcommand{\alexander}[1]{{\color{mygreen}#1}}

